Global Internet public peering capacity of interconnection: a complex network analysis

A massive and growing part of Autonomous System (AS)-level traffic exchanges takes place at Internet Exchange Points (IXPs). This paper leverages PeeringDB, a database providing a partial but reasonable view of the global interconnection of ASes at IXPs, to model a complex graph enabling the characterization of the key Internet peering players and their interactions over time. We model a PeeringDB snapshot as a weighted directed bipartite graph, called the pDB c-graph, that captures the port size ASes possess at IXPs using available metadata. This novel model of the Internet is shown to picture relevant features of a complex network that groups ASes and IXPs in geographical areas of influence. From this model, we extract central players of public peering such as hypergiant AS content providers and major regional traffic receivers. Most importantly, this graph model opens the way to apply spectral analysis using reduced Google matrix in order to retrieve the intensity of possible interactions between ASes on the basis of pure connectivity information. As an illustration, we retrieve the timely evolution of the peering network to show how the central content and cloud providers have increased their reach to eyeball networks during Covid-19 pandemic.

==> PRCR_dates_tab.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{tabular}{@{}lllll@{}}
\toprule
   & \begin{tabular}[c]{@{}l@{}}PageRank \\ 2020-01-01\end{tabular} & \begin{tabular}[c]{@{}l@{}}PageRank\\ 2020-06-01\end{tabular} & \begin{tabular}[c]{@{}l@{}}Reverse PageRank\\ 2020-01-01\end{tabular} & \begin{tabular}[c]{@{}l@{}}Reverse PageRank\\ 2020-06-01\end{tabular} \\ \midrule
0  & IX.br (PTT.br) São Paulo   & IX.br (PTT.br) São Paulo   & IX.br (PTT.br) São Paulo        & IX.br (PTT.br) São Paulo   \\
1  & DE-CIX Frankfurt         & DE-CIX Frankfurt        & DE-CIX Frankfurt                & DE-CIX Frankfurt           \\
2  & AMS-IX                   & AMS-IX                  & Facebook Inc                    & Facebook Inc               \\
3  & LINX LON1                & LINX LON1               & AMS-IX                          & AMS-IX                     \\
4  & Amazon.com               & Amazon.com              & Akamai Technologies             & Akamai Technologies        \\
5  & Equinix Singapore        & Equinix Singapore       & Google LLC                      & {\bf Netflix}                \\
6  & NAPAfrica IX Johannesburg& NAPAfrica IX Johannesburg  & LINX LON1                       & LINX LON1                  \\
7  & NL-ix                    & {\bf SIX Seattle}       & Netflix                         & Google LLC                 \\
8  & SIX Seattle              & {\bf IX.br (PTT.br) Rio de Janeiro}  & Apple Inc.       & {\bf Microsoft}          \\
9  & Equinix Ashburn          & NL-ix                   & Microsoft                       & Apple Inc.                 \\
10 & EPIX.Katowice            & EPIX.Katowice           & Amazon.com                      & {\bf Fastly, Inc.}          \\
11 & IX.br (PTT.br) Rio de Janeiro  & Equinix Ashburn         & StackPath (Highwinds)       & Amazon.com                 \\
12 & Hurricane Electric       & Hurricane Electric      & Cloudflare                      & StackPath (Highwinds)      \\
13 & Google LLC               & {\bf Equinix Chicago}  & Fastly, Inc.                    & Cloudflare                 \\
14 & Equinix Chicago          & Google LLC              & NL-ix                           & {\bf Equinix Singapore} \\
15 & Netnod Stockholm         & {\bf MIX-IT}        & Equinix Singapore           & {\bf Verizon Digital Media Services}\\
16 & TorIX                    & TorIX                   & NAPAfrica IX Johannesburg       & NAPAfrica IX Johannesburg  \\
17 & BBIX Tokyo               & {\bf Microsoft}      & Netnod Stockholm                & NL-ix                      \\
18 & Apple Inc.               & {\bf France-IX Paris}  & Equinix Ashburn                 & Equinix Ashburn            \\
19 & MIX-IT                   & {\bf HKIX}          & Verizon Digital Media Services      & {\bf SIX Seattle}     \\ \bottomrule
\end{tabular}


==> canny_tab.tex <==
%%Données de la soumission sigcomm
% \resizebox{.5\textwidth}{!}{%
% \begin{tabular}{@{\hskip 1pt}l@{\hskip 4pt}l@{\hskip 4pt}l@{\hskip 4pt}l@{\hskip 1pt}}
% \toprule
% Name          & Peak Dates                          & Peak Amplitude       & Delta \\ \midrule
% Africa        & {\bf 2020.02.15}, {\bf 2020.04.15}, 2019.09.15 & {\bf 0.132}, {\bf 0.125}, 0.102 & 39.01          \\
% South America & {\bf 2020.04.15}                           & {\bf 0.157}                 & 55.82          \\
% Australia     & {\bf 2020.04.15}, 2019.11.15              & {\bf 0.119}, 0.111         & 38.35          \\
% North America & {\bf 2020.04.15}, 2019.05.01              & {\bf 0.126}, 0.070         & 25.77          \\
% Asia Pacific  & {\bf 2020.04.15}, 2019.12.01, 2019.06.01 & {\bf 0.093}, 0.076, 0.072 & 25.80          \\
% Europe        & {\bf 2020.04.01}, 2019.11.01              & {\bf 0.114}, 0.106         & 18.57          \\\hline\hline
% Brazil            & {\bf 2020.04.15}, 2019.07.01              & {\bf 0.162}, 0.057         & 56.26          \\
% Spain            & {\bf 2020.03.15}, 2019.07.15, 2019.04.15 & {\bf 0.135}, 0.098, 0.072 & 38.21          \\
% Italy            & {\bf 2020.04.15}, 2019.10.01, 2019.05.15 & {\bf 0.140}, 0.084, 0.074 & 34.57          \\
% India            & 2020.05.15, 2019.04.01, 2019.07.15 & 0.113, 0.082, 0.082 & 45.27          \\
% Hong Kong            & {\bf 2020.03.15}, 2019.12.01, 2019.05.15 & {\bf 0.080}, 0.068, 0.054 & 24.85          \\
% USA            & {\bf 2020.04.15}, 2019.05.01              & {\bf 0.128}, 0.070         & 26.02          \\
% Singapore            & {\bf 2020.04.15}, 2019.11.15, 2019.05.01 & {\bf 0.104}, 0.088, 0.073 & 30.41          \\
% Poland            & {\bf 2020.04.01}, 2019.07.01, 2019.11.01 & {\bf 0.070}, 0.038, 0.037 & 21.49          \\
% Russia            & 2019.10.15, {\bf 2020.04.15}, 2020.07.01 & {\bf 0.120}, 0.104, 0.099 & 30.71          \\
% France            & {\bf 2020.02.15}, 2019.05.15              & {\bf 0.139}, 0.090         & 19.88          \\
% GB            & {\bf 2020.03.15}, 2019.11.01, 2019.04.15 & {\bf 0.124}, 0.122, 0.071 & 17.63          \\
% Germany            & {\bf 2020.04.01}, 2019.11.15, 2019.08.15 & {\bf 0.087}, 0.077, 0.074 & 15.02           \\
% Netherlands            & 2019.06.15, {\bf 2020.05.01}, 2019.11.15 & 0.117, {\bf 0.097}, 0.088 & 12.49           \\\hline\hline
% Netflix       & {\bf 2020.03.15}, 2019.05.01              & {\bf 0.212}, 0.071         & 69.26          \\
% Microsoft     & {\bf 2020.04.01}, 2019.11.01, 2019.06.01 & {\bf 0.135}, 0.118, 0.099 & 42.27          \\
% Hurricane E.  & 2020.02.01, 2019.07.15              & 0.165, 0.108         & 17.69          \\
% Facebook      & {\bf 2020.03.15}, 2019.02.15              & {\bf 0.168}, 0.050         & 15.18          \\
% Akamai        & 2020.06.15, 2019.10.15, {\bf 2020.02.15} & 0.129, 0.120, {\bf 0.093} & 37.43          \\
% Apple Inc.    & {\bf 2020.03.15}, 2019.05.15              & {\bf 0.144}, 0.132         & 7.16           \\
% Google LLC    & 2019.10.15, 2019.04.01, 2020.06.15 & 0.165, 0.089, 0.057 & 11.09           \\ \bottomrule
% \end{tabular}
% }
%%Données de la soumission IMC2021
\resizebox{.48\textwidth}{!}{%
\begin{tabular}{@{\hskip 1pt}l|@{\hskip 4pt}c@{\hskip 4pt}|c@{\hskip 4pt}|l@{\hskip 1pt}}
\toprule
Name          & Peak dates                           & Peak amplitudes       & Delta \\ \midrule
Africa        & \textbf{2020-05-01} | \textbf{2020-02-15} | 2020-11-01 & \textbf{0.104} | \textbf{0.104} | 0.086 & 55.66 \\
South America & \textbf{2020-05-01} | 2020-09-01              & \textbf{0.107} | 0.106         & 100.12 \\
Australia     & 2020-08-15 | 2019-11-15 | 2021-02-01 & 0.118 | 0.078 | 0.044 & 61.34 \\
North America & \textbf{2020-05-01} | 2020-10-15 | 2019-05-01 & \textbf{0.097} | 0.088 | 0.048 & 44.27 \\
Asia Pacific  & 2020-11-01 | 2020-07-15 | 2019-12-15 & 0.087 | 0.082 | 0.055 & 54.05 \\
Europe        & 2020-12-01 | \textbf{2020-04-01} | 2019-11-01 & 0.093 | \textbf{0.079} | 0.068 & 38.98 \\
BR            & \textbf{2020-05-01} | 2020-09-01 | 2019-07-15 & \textbf{0.113} | 0.109 | 0.035 & 97.45 \\
ES            & \textbf{2020-03-15} | 2020-10-15 | 2019-07-15 & \textbf{0.094} | 0.071 | 0.065 & 69.47 \\
IT            & \textbf{2020-05-01} | 2020-11-15 | 2019-10-01 & \textbf{0.112} | 0.077 | 0.062 & 51.71 \\
IN            & 2020-10-15 | 2019-04-01 | 2019-07-15 & 0.110 | 0.042 | 0.042 & 115.17 \\
HK            & \textbf{2020-03-15} | 2020-12-01 | 2019-05-15 & \textbf{0.084} | 0.065 | 0.054 & 44.24 \\
US            & \textbf{2020-05-01} | 2020-10-15 | 2019-05-01 & \textbf{0.099} | 0.088 | 0.049 & 44.38 \\
SG            & 2020-08-01 | 2020-12-01 | 2019-11-15 & 0.094 | 0.079 | 0.060 & 55.56 \\
PL            & 2020-12-01 | \textbf{2020-04-15} | 2019-07-01 & 0.086 | \textbf{0.075} | 0.038 & 46.84 \\
RU            & 2020-12-01 | 2020-08-15 | 2019-10-15 & 0.113 | 0.091 | 0.065 & 74.57 \\
FR            & 2020-12-15 | \textbf{2020-02-15} | 2019-05-15 & 0.098 | \textbf{0.092} | 0.058 & 44.80 \\
GB            & \textbf{2020-04-01} | 2019-11-01 | 2020-06-15 & \textbf{0.099} | 0.093 | 0.088 & 26.54 \\
DE            & \textbf{2020-04-01} | 2020-09-15 | 2019-11-15 & \textbf{0.089} | 0.077 | 0.073 & 26.29 \\
NL            & 2020-11-15 | 2019-06-15 | \textbf{2020-05-15} & 0.097 | 0.077 | \textbf{0.075} & 28.45 \\
Netflix       & \textbf{2020-04-01} | 2019-05-01              & \textbf{0.170} | 0.056         & 88.46 \\
Microsoft     & \textbf{2020-04-15} | 2020-11-15 | 2019-11-01 & \textbf{0.101} | 0.096 | 0.083 & 77.54 \\
Hurricane E.  & 2020-10-01 | \textbf{2020-02-15} | 2019-07-15 & 0.111 | \textbf{0.085} | 0.053 & 44.93 \\
Facebook      & 2020-12-01 | \textbf{2020-03-15} | 2019-02-15 & 0.153 | \textbf{0.084} | 0.023 & 42.57 \\
Akamai        & 2020-07-01 | 2020-11-01 | 2019-10-15 & 0.106 | 0.088 | 0.078 & 75.74 \\
Apple Inc.    & \textbf{2020-03-15} | 2019-05-15 | 2021-02-15 & \textbf{0.144} | 0.132 | 0.021 & 7.16  \\
Google LLC    & 2020-11-15 | 2019-10-15 | 2019-04-01 & 0.157 | 0.082 | 0.044 & 49.89 \\ \bottomrule
\end{tabular}
}

==> catchers_tab_horizontal.tex <==
%%horizontal double column
\resizebox{.98\textwidth}{!}{%
\begin{tabular}{@{}lllllllllllll@{}}
\toprule
PageRank & US & BR & FR & DE & GB & IT & ES & RU & PL & IN & HK & SG           \\ \midrule
1 &
  T-Mobile USA &
  G8 &
  SFR Group &
  Telefónica Germany GmbH \& Co. OHG &
  TalkTalk &
  NGI &
  Vodafone España &
  RASCOM &
  VECTRA &
  Excitel &
  Viettel &
  Indosat Ooredoo \\
2 &
  Claro S.A. &
  Claro S.A. (NET) &
  Zayo France &
  Vodafone Germany &
  Sky Broadband &
  Fastweb &
  Aire Networks del Mediterraneo &
  Delta Telecom &
  Polkomtel Sp. z o.o. &
  Sify Technologies Limited &
  VNPT &
  DTAC IIG \\
3 &
  Zayo (Abovenet Communications Inc.) &
  Angola Cables &
  moji &
  Saudi Telecom Company (STC IGW) &
  Hyperoptic &
  Vodafone Italy &
  TVHoradada &
  Kaztranscom &
  Orange Polska S.A. (IX) &
  Esto Broadband &
  HKT Limited &
  MyRepublic Ltd \\
4 &
  i3D.net &
  Algar Telecom &
  &
  1\&1 Versatel Deutschland GmbH &
  &
  &
  Digi Spain Telecom &
  Dataline Net &
  &
  Indusind Media and Communication Ltd &
  HGC &
  PT Mora Telematika Indonesia \\
5        &    &    &    &    &    &    &    &    &    &    &    & CBN Networks \\ \bottomrule
\end{tabular}}

==> catchers_tab_vertical.tex <==
%%vertical single column -
% \begin{tabular}{@{}ll@{}}
% \toprule
% Code & Name                                 \\ \midrule
% US0  & Verisign                             \\
% US1  & T-Mobile USA                         \\
% US2  & Claro S.A.                           \\
% US3  & Zayo (Abovenet Communications Inc.)  \\
% US4  & i3D.net                              \\
% BR0  & Open X Tecnologia Ltda               \\
% BR1  & G8                                   \\
% BR2  & Claro S.A. (NET)                     \\
% BR3  & Angola Cables                        \\
% BR4  & Algar Telecom                        \\
% FR0  & Bouygues Telecom ISP                 \\
% FR1  & SFR Group                            \\
% FR2  & Zayo France                          \\
% FR3  & moji                                 \\
% DE0  & Core-Backbone                        \\
% DE1  & Telefónica Germany GmbH \& Co. OHG   \\
% DE2  & Vodafone Germany                     \\
% DE3  & Saudi Telecom Company (STC IGW)      \\
% DE4  & 1\&1 Versatel Deutschland GmbH       \\
% GB0  & BTnet (BT's UK IP Network - AS2856)  \\
% GB1  & TalkTalk                             \\
% GB2  & Sky Broadband                        \\
% GB3  & Hyperoptic                           \\
% IT0  & WIND Telecomunicazioni S.p.A.        \\
% IT1  & NGI                                  \\
% IT2  & Fastweb                              \\
% IT3  & Vodafone Italy                       \\
% ES0  & MásMóvil                             \\
% ES1  & Vodafone España                      \\
% ES2  & Aire Networks del Mediterraneo       \\
% ES3  & TVHoradada                           \\
% ES4  & Digi Spain Telecom                   \\
% RU0  & ER-Telecom                           \\
% RU1  & RASCOM                               \\
% RU2  & Delta Telecom                        \\
% RU3  & Kaztranscom                          \\
% RU4  & Dataline Net                         \\
% PL0  & Netia S.A.                           \\
% PL1  & VECTRA                               \\
% PL2  & Polkomtel Sp. z o.o.                 \\
% PL3  & Orange Polska S.A. (IX)              \\
% IN0  & Ani Network                          \\
% IN1  & Excitel                              \\
% IN2  & Sify Technologies Limited            \\
% IN3  & Esto Broadband                       \\
% IN4  & Indusind Media and Communication Ltd \\
% HK0  & Hong Kong Broadband Network LTD      \\
% HK1  & Viettel                              \\
% HK2  & VNPT                                 \\
% HK3  & HKT Limited                          \\
% HK4  & HGC                                  \\
% SG0  & True Internet Corporation            \\
% SG1  & Indosat Ooredoo                      \\
% SG2  & DTAC IIG                             \\
% SG3  & MyRepublic Ltd                       \\
% SG4  & PT Mora Telematika Indonesia         \\
% SG5  & CBN Networks                         \\ \bottomrule
% \end{tabular}

%%vertical doubled
\resizebox{.48\textwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
Code & Name                                & Code & Name                                 \\ \midrule
US1  & \textbf{Verisign}                            & ES3  & \textbf{Aire Networks del M.}       \\
US2  & T-Mobile                      & ES4  & TVHoradada                           \\
US3  & \textbf{Claro}                           & ES5  & Digi Spain Telecom                   \\
US4  & \textbf{Zayo}  & RU1  & \textbf{ER-Telecom}                           \\
US5  & \textbf{i3D.net}                             & RU2  & \textbf{RASCOM}                               \\
BR1  & \textbf{Open X Tecnologia}              & RU3  & \textbf{Delta Telecom}                        \\
BR2  & \textbf{G8}                                  & RU4  & \textbf{Kaztranscom}                          \\
BR3  & Claro (NET)                   & RU5  & \textbf{Dataline Net}                         \\
BR4  & \textbf{Angola Cables}                       & PL1  & \textbf{Netia}                           \\
BR5  & \textbf{Algar Telecom}                       & PL2  & VECTRA                               \\
FR1  & Bouygues Telecom                & PL3  & Polkomtel                  \\
FR2  & SFR Group                           & PL4  & \textbf{Orange Polska}              \\
FR3  & \textbf{Zayo France}                         & IN1  & Ani Network                          \\
FR4  & moji                                & IN2  & Excitel                              \\
DE1  & \textbf{Core-Backbone}                       & IN3  & \textbf{Sify Technologies}            \\
DE2  & \textbf{Telefónica Germany}  & IN4  & Esto Broadband                       \\
DE3  & Vodafone Germany                    & IN5  & Indusind Media and Com. \\
DE4  & \textbf{Saudi Telecom Company}     & HK1  & Hong Kong Broadband Network      \\
DE5  & 1\&1 Versatel Deutschland      & HK2  & Viettel                              \\
GB1  & \textbf{BTnet}  & HK3  & VNPT                                 \\
GB2  & TalkTalk                            & HK4  & HKT                         \\
GB3  & Sky Broadband                       & HK5  & \textbf{HGC}                                  \\
GB4  & Hyperoptic                          & SG1  & \textbf{True Internet Corporation}            \\
IT1  & \textbf{WIND Telecom.}       & SG2  & \textbf{Indosat Ooredoo}                      \\
IT2  & NGI                                 & SG3  & DTAC IIG                             \\
IT3  & Fastweb                             & SG4  & MyRepublic                      \\
IT4  & \textbf{Vodafone Italy}                      & SG5  & \textbf{PT Mora Telematika Indonesia}         \\
ES1  & MásMóvil                            & SG6  & \textbf{CBN Networks}                         \\
ES2  & Vodafone España                     &      &                                      \\ \bottomrule
\end{tabular}}



==> louvain_tab.tex <==
\begin{tabular}{@{}cccccc@{}}
\toprule
\begin{tabular}{c} Louvain\\Cluster\end{tabular}   & IXPs country distribution               & \begin{tabular}{c}\#Different \\IXP countries\end{tabular}   & Grouping interpretation   & Port capacity (\%) & \# of IXP (\%) \\ \midrule
0  & US: 74 | CA: 12 | CO: 2 | GU: 2 | SG: 2 & 13 & North America          & 18.5 & 14.6 \\
1  & DE: 22 | AT: 4 | CH: 4 | US: 2 | AE: 1  & 16 & Germanic countries     & 11.7 & 6.4  \\
2  & FR: 15 | GB: 11 | IE: 4 | US: 3 | AU: 2 & 16 & Western Europe         & 10.1 & 6.9  \\
4  & NL: 9 | BE: 1 | BJ: 1 | CA: 1 | IS: 1   & 6  & Netherlands            & 10.1 & 2.0  \\
7  & BR: 34 | RO: 4 | AO: 2 | KE: 2 | US: 2  & 11 & Brazil                 & 8.6  & 7.3  \\
8  & AR: 22 | JP: 13 | CL: 6 | HK: 2 | BH: 1 & 10 & South America, East Asia                      & 8.3  & 7.1  \\
5  & ID: 16 | TH: 7 | PH: 4 | HK: 3 | SG: 3  & 12 & South-East Asia           & 7.1  & 6.3  \\
10 & RU: 30 | UA: 12 | BG: 6 | KZ: 3 | KG: 2 & 12                        & Eastern Europe & 5.9                & 9.0                \\
3  & SE: 10 | NO: 7 | ES: 6 | FI: 4 | DK: 3  & 15 & Scandinavian countries & 5.0  & 6.7  \\
9  & AU: 21 | NZ: 6 | US: 4 | MY: 1          & 4  & Oceania Pacific        & 3.4  & 4.7  \\
6  & TZ: 5 | ZA: 5 | US: 4 | CA: 2 | CD: 2   & 36 & Africa                 & 2.8  & 7.3  \\
14 & PL: 11 | RO: 2 | PH: 1                  & 3  & Eastern Europe         & 2.3  & 2.0  \\ \bottomrule
\end{tabular}




% June
% \begin{tabular}{@{}lllllllllllll@{}}
% \resizebox{.98\textwidth}{!}{%
% \begin{tabular}{@{}lcccccccccccc@{}}
% \toprule
%  &
%   1 &
%   0 &
%   7 &
%   5 &
%   2 &
%   10 &
%   13 &
%   3 &
%   11 &
%   6 &
%   9 &
%   15 \\ \midrule
% IXPs country distribution &
%   \begin{tabular}{llll}&DE: 18 &NL: 9\\ &AT: 4 &CH: 2 \end{tabular}&
%   \begin{tabular}{llll}&US: 65 &CA: 12\\ &ES: 2 &GR: 2 \end{tabular}&
%   \begin{tabular}{llll}&BR: 36 &BG: 5\\ &CL: 5 &RO: 4 \end{tabular}&
%   \begin{tabular}{llll}&ID: 16 &PH: 5\\ &BD: 3 &HK: 3 \end{tabular}&
%   \begin{tabular}{llll}&GB: 13 &IE: 5\\ &US: 3 &CH: 1 \end{tabular}&
%   JP: 12 &
%   \begin{tabular}{llll}&RU: 32 &UA: 15\\ &LT: 4 &LV: 3 \end{tabular}&
%   \begin{tabular}{llll}&SE: 17 &FI: 7\\ &NO: 6  &AU: 5 \end{tabular}&
%   \begin{tabular}{llll}&AU: 24 &NZ: 7\\ &US: 6 &CA: 1 \end{tabular}&
%   \begin{tabular}{llll}&ZA: 7 &TZ: 5\\ &US: 3 &LB: 2  \end{tabular}&
%   \begin{tabular}{llll}&FR: 13 &BE: 2\\ &LU: 2 &DJ: 1 \end{tabular}&
%   \begin{tabular}{llll}&CZ: 5 &TH: 4\\ &SK: 3 \end{tabular}\\
% \#Different IXP countries &
%   14 &
%   18 &
%   16 &
%   10 &
%   9 &
%   1 &
%   11 &
%   10 &
%   6 &
%   37 &
%   6 &
%   3 \\
% Grouping interpretation &
%   \begin{tabular}{cc}&Germanic\\&countries \end{tabular}&
%   North America &
%   Brazil &
%   Asia Pacific &
%   British Isles &
%   Japan &
%   \begin{tabular}{cc}&Former western\\&USSR members \end{tabular} &
%   \begin{tabular}{cc}&Scandinavian\\&countries \end{tabular}&
%   Oceania Pacific &
%   Africa &
%   \begin{tabular}{cc}&French speaking\\&Countries \end{tabular} &
%   Central Europe \\
% Port capacity (\%) &
%   19.6 &
%   19.3 &
%   11.5 &
%   6.8 &
%   6.5 &
%   6.2 &
%   5.2 &
%   4.1 &
%   3.5 &
%   2.6 &
%   2.4 &
%   2.4 \\
% Number of IXP (\%) &
%   5.9 &
%   13.1 &
%   9.1 &
%   5.7 &
%   3.7 &
%   1.6 &
%   8.7 &
%   6.3 &
%   5.4 &
%   6.8 &
%   2.7 &
%   1.6 \\ \bottomrule
% \end{tabular}
% }

%January
% \resizebox{1.\textwidth}{!}{%
% \begin{tabular}{lcccccc}
% \toprule
%  &
%   0 &
%   1 &
%   2 &
%   4 &
%   7 &
%   8 \\ \midrule
%  % 5 &
%  % 10 &
%  % 3 &
%  % 9 &
%  % 6 &
%  % 14 \\ \midrule
%   \begin{tabular}{c}IXP countries\\ distribution \end{tabular}&
%   \begin{tabular}{llll}&US: 74 &CA: 12\\ &CO: 2 &GU: 2 \end{tabular}&
%   \begin{tabular}{llll}&DE: 22 &AT: 4\\ &CH: 4 &US: 2 \end{tabular}&
%   \begin{tabular}{llll}&FR: 15 &GB: 11\\ &IE: 4 &US: 3 \end{tabular}&
%   \begin{tabular}{llll}&NL: 9 &BE: 1\\ &BJ: 1 &CA: 1 \end{tabular}&
%   \begin{tabular}{llll}&BR: 34 &RO: 4\\ &AO: 2 &KE: 2 \end{tabular}\\
%  % \begin{tabular}{llll}&AR: 22 &JP: 13\\ &CL: 6 &HK: 2 \end{tabular}&
%  % \begin{tabular}{llll}&ID: 16 &TH: 7\\ &PH: 4 &HK: 3 \end{tabular}&
%  % \begin{tabular}{llll}&RU: 30 &UA: 12\\ &BG: 6 &KZ: 3 \end{tabular}&
%  % \begin{tabular}{llll}&SE: 10 &NO: 7\\ &ES: 6  &FI: 4 \end{tabular}&
%  % \begin{tabular}{llll}&AU: 21 &NZ: 6\\ &US: 4 &MY: 1 \end{tabular}&
%  % \begin{tabular}{llll}&TZ: 5 &ZA: 5\\ &US: 4 &CD: 2  \end{tabular}&
%  % \begin{tabular}{llll}&PL: 11 &RO: 2\\ &PH: 1  \end{tabular} \\
  
 
% \begin{tabular}{c}\#Different\\ IXP countries \end{tabular}&
%   13 &
%   16 &
%   16 &
%   6 &
%   11 &
%   10 \\
%  % 12 &
%  % 12 &
%  % 15 &
%  % 4 &
%  % 36 &
%  % 3 \\
% \begin{tabular}{c}Cluster\\ Interpretation  \end{tabular}&
%   North America &
%   \begin{tabular}{cc}&Germanic\\&countries \end{tabular}&
%   \begin{tabular}{cc}&Western\\&Europe \end{tabular}&
%   Netherlands &
%   Brazil &
%   \begin{tabular}{cc}&South America\\& East Asia \end{tabular} \\
   
%   %\begin{tabular}{cc}&South-East\\&Asia \end{tabular}&
%   %\begin{tabular}{cc}&Eastern\\&Europe \end{tabular} &
%   %\begin{tabular}{cc}&Scandinavian\\&countries \end{tabular}&
%   %Oceania Pacific &
%   %Africa &
%   %Poland \\
% Port capacity (\%) &
%   18.5 &
%   11.7 &
%   10.1 &
%   10.1 &
%   8.6 &
%   8.3 \\
%  % 7.1 &
%  % 5.9 &
%  % 5.0 &
%  % 3.4 &
%  % 2.8 &
%  % 2.3 \\
% Number of IXP (\%) &
%   14.6 &
%   6.4 &
%   6.9 &
%   2.0 &
%   7.3 &
%   7.1 \\ \bottomrule
% %  6.3 &
% %  9.0 &
% %  6.7 &
% %  4.7 &
% %  7.3 &
% %  2.0 \\ \bottomrule
% \end{tabular}
% }

% \resizebox{1.\textwidth}{!}{%
% \begin{tabular}{lcccccc}
% \toprule
%  &
%   5 &
%   10 &
%   3 &
%   9 &
%   6 &
%   14 \\ \midrule
%   \begin{tabular}{c}IXP countries\\ distribution \end{tabular}&
%   \begin{tabular}{llll}&AR: 22 &JP: 13\\ &CL: 6 &HK: 2 \end{tabular}&
%   \begin{tabular}{llll}&ID: 16 &TH: 7\\ &PH: 4 &HK: 3 \end{tabular}&
%   \begin{tabular}{llll}&RU: 30 &UA: 12\\ &BG: 6 &KZ: 3 \end{tabular}&
%   \begin{tabular}{llll}&SE: 10 &NO: 7\\ &ES: 6  &FI: 4 \end{tabular}&
%  \begin{tabular}{llll}&AU: 21 &NZ: 6\\ &US: 4 &MY: 1 \end{tabular}&
%   \begin{tabular}{llll}&TZ: 5 &ZA: 5\\ &US: 4 &CD: 2  \end{tabular}&
%   \begin{tabular}{llll}&PL: 11 &RO: 2\\ &PH: 1  \end{tabular} \\
%   \begin{tabular}{c}\#Different\\ IXP countries \end{tabular}&
%   12 &
%  12 &
%   15 &
%   4 &
%   36 &
%   3 \\


